MissDDIM: Deterministic and Efficient Conditional Diffusion for Tabular Data Imputation

Diffusion models have recently emerged as powerful tools for missing data imputation by modeling the joint distribution of observed and unobserved variables. However, existing methods, typically based on stochastic denoising diffusion probabilistic models (DDPMs), suffer from high inference latency and variable outputs, limiting their applicability in real-world tabular settings. To address these deficiencies, we present in this paper MissDDIM, a conditional diffusion framework that adapts Denoising Diffusion Implicit Models (DDIM) for tabular imputation. While stochastic sampling enables diverse completions, it also introduces output variability that complicates downstream processing.

==> plot1.tex <==
\begin{figure}[!ht]
\centering
\definecolor{colA}{HTML}{264653}
\definecolor{colB}{HTML}{287271}
\definecolor{colC}{HTML}{2A9D8F}
\definecolor{colD}{HTML}{8AB17D}
\definecolor{colE}{HTML}{BABB74}
\definecolor{colF}{HTML}{E9C46A}
\definecolor{colG}{HTML}{EFB366}
\definecolor{colH}{HTML}{F4A261}
\definecolor{colI}{HTML}{EE8959}
\definecolor{colJ}{HTML}{E76F51}
\definecolor{colK}{HTML}{F94144}
% Style
\pgfplotsset{
    every axis plot/.append style={thick},
    cycle list={
        {colA, dashed, mark=+},
        {colB, dashed, mark=halfcircle*},
        {colC, dashed, mark=x},
        {colD, dashed, mark=star},
        {colE, dashed, mark=-},
        {colF, solid, mark=*}, %target
        {colG, dashed, mark=+},
        {colH, dashed, mark=halfcircle*},
        {colI, dashed, mark=x},
        {colJ, dashed, mark=star},
        {colK, dashed, mark=-}
    }
}
% 15 datasets for 5 x 3 layout
\hspace*{-4em}
\foreach \dataset [count=\i] in {MCAR,MAR, MNAR,
MCAR,MAR, MNAR,  
MCAR,MAR, MNAR, 
MCAR,MAR, MNAR,
MCAR,MAR, MNAR } {
  \begin{subfigure}[t]{0.23\textwidth}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        grid=both,
        grid style={dashed, gray!40},
        % Title only in first row
        title={\ifnum\i<4 \dataset \fi},
        title style={font=\small, yshift=-1.2ex},
        % X label only in last row
        xlabel={\ifnum\i>12 Missing Rate    \fi},
        ylabel={\ifnum\i=1 Banknote \else \ifnum\i=4 California \else \ifnum\i=7 Letter \else \ifnum\i=10 Adult \else \ifnum\i=13 Student \fi\fi\fi\fi\fi},
        xmin=0.05, xmax=0.75,
        ymin=0.15, ymax=0.35,
        xtick={0.1,0.3,0.5,0.7},
        ytick={0.15,0.2,0.25,0.3,0.35},
        tick label style={font=\tiny},
        label style={font=\small},
        title style={font=\small},
        width=\textwidth,
        height=0.7\textwidth,
        y label style={at={(axis description cs:0.5,.5)},anchor=south},
        x label style={at={(axis description cs:0.5,-0.1)},anchor=south},
        yticklabels={\ifnum\i=1 \else \ifnum\i=6 \else \ifnum\i=11 \else \empty \fi\fi\fi},
        enlargelimits=false,
        legend style={at={(0.5,-10)}, anchor=north, 
        scale=0.8,  
        font=\small, cells={anchor=west}, /tikz/every even column/.style={column sep=0.6em}},
        legend columns=6,
         legend entries={Mean,MICE,GAIN,MWAE,GRAPE,IVGAE,KNN,MisF,NMWAE,HIVAE,IGRM},
        legend to name=sharedlegend
    ]
    % Dummy plots
    \addplot+[colA] coordinates {(0.1,0.22) (0.3,0.24) (0.5,0.26) (0.7,0.29)};
    \addplot+[colC] coordinates {(0.1,0.21) (0.3,0.23) (0.5,0.26) (0.7,0.28)};
    \addplot+[colE] coordinates {(0.1,0.19) (0.3,0.21) (0.5,0.24) (0.7,0.26)};
    \addplot+[colG] coordinates {(0.1,0.17) (0.3,0.19) (0.5,0.21) (0.7,0.23)};
    \addplot+[colI] coordinates {(0.1,0.20) (0.3,0.22) (0.5,0.23) (0.7,0.25)};
    \addplot+[colK] coordinates {(0.1,0.18) (0.3,0.20) (0.5,0.21) (0.7,0.23)};
    \addplot+[colB] coordinates {(0.1,0.20) (0.3,0.22) (0.5,0.25) (0.7,0.27)};
    \addplot+[colD] coordinates {(0.1,0.19) (0.3,0.21) (0.5,0.23) (0.7,0.25)};
    \addplot+[colF] coordinates {(0.1,0.18) (0.3,0.21) (0.5,0.22) (0.7,0.24)};
    \addplot+[colH] coordinates {(0.1,0.16) (0.3,0.18) (0.5,0.20) (0.7,0.22)};
    \addplot+[colJ] coordinates {(0.1,0.15) (0.3,0.17) (0.5,0.19) (0.7,0.21)};
    % Legend only in the last subplot
    \ifnum\i=15
        \addlegendentry{Mean}
        \addlegendentry{MICE}
        \addlegendentry{GAIN}
        \addlegendentry{HIVAE}
        \addlegendentry{MIWAE}
        \addlegendentry{MissDDIM}
        \addlegendentry{TabCSDI}
        \addlegendentry{KNN}
        \addlegendentry{MisF}
        \addlegendentry{MIWAE}
        \addlegendentry{GRAPE}
        \addlegendentry{MissDiff}
        
    \fi
    \end{axis}
    \end{tikzpicture}
  \end{subfigure}%
  \hspace*{-4.5em} 
  \ifnum\i=3 \par\vspace{-2em}\hspace*{-4em} \fi
  \ifnum\i=6 \par\vspace{-2em}\hspace*{-4em}\fi
  \ifnum\i=9 \par\vspace{-2em}\hspace*{-4em}\fi
  \ifnum\i=12 \par\vspace{-2em}\hspace*{-3.2em}\fi
}
\vspace{-1em}
\begin{center}
\scalebox{0.8}{  % ⬅️ 缩放比例（比如 80%）
  \ref{sharedlegend}
}
\end{center}
\caption{RMSE across different missing rates for various imputation methods under three missing data mechanisms.}
\end{figure}




